AI-enabled Automation for Completeness Checking of Privacy Policies

Technological advances in information sharing have raised concerns about data protection. Privacy policies contain privacy-related requirements about how the personal data of individuals will be handled by an organization or a software system (e.g., a web service or an app). In Europe, privacy policies are subject to compliance with the General Data Protection Regulation (GDPR). A prerequisite for GDPR compliance checking is to verify whether the content of a privacy policy is complete according to the provisions of GDPR. Incomplete privacy policies might result in large fines on violating organization as well as incomplete privacy-related software specifications. Manual completeness checking is both time-consuming and error-prone. In this paper, we propose AI-based automation for the completeness checking of privacy policies. Through systematic qualitative methods, we first build two artifacts to characterize the privacy-related provisions of GDPR, namely a conceptual model and a set of completeness criteria. Then, we develop an automated solution on top of these artifacts by leveraging a combination of natural language processing and supervised machine learning. Specifically, we identify the GDPR-relevant information content in privacy policies and subsequently check them against the completeness criteria. To evaluate our approach, we collected 234 real privacy policies from the fund industry. Over a set of 48 unseen privacy policies, our approach detected 300 of the total of 334 violations of some completeness criteria correctly, while producing 23 false positives. The approach thus has a precision of 92.9% and recall of 89.8%. Compared to a baseline that applies keyword search only, our approach results in an improvement of 24.5% in precision and 38% in recall.

==> approach-backup.tex <==
\section{AI-based Completeness Checking approach (RQ3)} \label{sec:approach}

\begin{figure*}[ht!]
\centering
\includegraphics[width=0.75\linewidth] {img/tool}
\caption{Overview of the Completeness Checking Approach (CompAI).} \label{fig:approach}
%\vspace*{-1.7em}
\end{figure*}

In this section, we address RQ3 and present our AI-based approach for checking the completeness of privacy policies against GDPR (thereafter referred to as \textit{CompAI}). 
\textcolor{blue}{We note that our approach does not apply sophisticated deep learning methods because we do not have enough data.}
%Our overall approach
CompAI, as shown in Fig.~\ref{fig:approach}, is composed of two main phases.  %, namely metadata identification and compliance checking. %as depicted in
Phase~A, \textit{metadata identification}, takes as an input a privacy policy, and returns the metadata types that are present in this policy as an intermediary output.
Phase~B, \textit{completeness checking}, takes as an input the identified metadata types from Phase~A and the user input based on the questionnaire (explained in Sec.~\ref{sec:criteria}). Phase~B then returns a detailed report about whether the input privacy policy is complete according to GDPR.  
We elaborate  these two phases next. 

\subsection{Metadata Identification (Phase~A)} 
Phase~A uses a combination of NLP and ML to identify the metadata types that are present in a given privacy policy. 
%Recall from Sec.~\ref{sec:qualitative} the three levels of metadata types in our conceptual model (Figure~\ref{fig:metadata}), \textit{level-1}, \textit{level-2} and \hbox{\textit{level-3}}. 
Our metadata identification approach aims to solve a hierarchical, multi-label and multi-class classification problem. The nature of the problem is visible from the conceptual model in Fig.~\ref{fig:metadata}, where most level-1 metadata types are further classified into sub-metadata types (level-2 and level-3). Multi-label classification reflects the fact that a sentence in the privacy policy can discuss one or more metadata types. Therefore, our solution can predict one or more potential labels (metadata types) for each sentence in the input privacy policy.
%i.e., each sentence in the input privacy policy is classified into one (or more) of the metadata types the are predicted to be present in that sentence.  
Our approach considers \textit{sentences} as the units of analysis. 
A sentence refers to the textual entity that results from applying the sentence splitting module in the NLP pipeline (Fig.~\ref{fig:pipeline}), irrespective of whether the sentence identified by this module corresponds to a grammatical sentence. 
The rationale behind using sentences rather than phrases %as units of analysis 
is that the former are more likely to contain the context necessary for understanding their meaning~\cite{michaelis:03} and thus lead to more accurate classification results. 

%To facilitate discussion throughout this section, we refer to three levels of metadata types, \textit{level-1}, \textit{level-2} and \hbox{\textit{level-3}}, as introduced in Sec.~\ref{sec:qualitative}.
%As depicted in Figure~\ref{fig:approach}, the metadata identification component takes as input a privacy policy and returns as output metadata annotations for each sentence in the input privacy policy. The component contains eight steps. 
%Our %metadata identification approach
Phase A is further composed of seven steps. In the first two steps, 
the text of the input privacy policy is preprocessed, generalized and transformed into a mathematical representation. 
In steps~3-5, we classify the sentences of the input privacy policy into one or more metadata types using three classification methods based on ML, semantic similarity, and keywords. \textcolor{blue}{As we will see, relying on these different and complementary methods is necessary to overcome the complexity of the hierarchical classification problem. }%(conceptual) model. 
In step~6, we combine the results of steps 3, 4, and 5 in order to predict metadata types for each sentence in the input privacy policy. In the last step, we refine the results through  post-processing. Steps are explained in detail next.
%ML-based classifiers. Each classifier in this step is a predictor for the presence of a certain level-1 or level-2 metadata type in sentences.
%In Step~4, we classify the sentences by analyzing how similar each sentence in the input privacy policy is to the groups of sentences annotated with level-2 metadata types. %level-2 metadata type groups in the training set described in Section~\ref{subsection:annotation}.  %Note that Step~5 does \emph{not} use the predictions of the classifiers built in Step~4. 
%In Step 5, we classify the sentences based on looking up pre-defined keywords and focusing on the metadata types at level-1, level-2 and level-3.

\subsubsection{Text Preprocessing and Generalization (Step~1)}
In step~1, we apply the NLP pipeline (Fig.~\ref{fig:pipeline}) %(as explained in Sec.~\ref{subsec:nlp}). %
to parse the input privacy policy and obtain the sentences. Using the annotations produced by the NLP pipeline, we then generalize the text in each sentence by  
%Text generalization is the task of 
replacing specific textual entities with more generic ones. 
More precisely, we replace named entities (as identified by the named entity recognizer in Fig.~\ref{fig:pipeline}) with their types. For example, the entities ``Japan'' and ``Hikari Bank Ltd'' in Fig.~\ref{fig:step1} will be replaced with the types \textit{location} and \textit{organization}, respectively. Similarly, we generalize emails, postal addresses, telephone numbers, and websites, e.g., the email address ``info@hikari.jp'' is replaced with \textit{email}. 
The intuition behind generalization is to normalize the text such that, despite the diversity across privacy policies we use for training (e.g., the mention of different locations), the approach can still learn common patterns and predict metadata types with high accuracy. 
The generalized sentences are further normalized through lemmatization and stopword removal, e.g., ``accepting'' (in Fig.~\ref{fig:step1}) becomes ``accept'' and the stopword ``by'' is removed. 

\begin{figure}[H]
\centering
\vspace*{-1em}
\includegraphics[width=\linewidth] {img/step1.pdf}
\vspace*{-1.8em}
\caption{Example of Text Preprocessing and Generalization.} \label{fig:step1}
\vspace*{-.5em}
\end{figure}

%, we apply a named entity recognizer to obtain annotations for \textit{organizations} and \textit{locations} in the text. 
%These two are named entities that appear frequently in privacy policies. 
%For example, if the text contains the country name \textit{United Kingdom}, then this is annotated as \textit{location}, whereas the company name \textit{Google LLC} is recognized as an \textit{organization}.

%\subsubsection{Text Generalization}
%For example, the country name \textit{United Kingdom} and the company name \textit{Google LLC} will be replaced by \textit{location} and  \textit{organization}, respectively. 

\subsubsection{Vectorization (Step~2)}
Step~2 transforms the textual sentences resulting from step~1 into embeddings. To do this, we utilize the pre-trained word-vector model of 100-dimensional vectors from GloVe~\cite{pennington:14} (introduced in  Sec.~\ref{subsec:embeddings}). \textcolor{blue}{Using off-the-shelf pre-trained word vectors is advantageous because our approach does not require extra training (in this step) to be extended for checking completeness of privacy policies from sectors other than fund.} 
%This model represents 100-dimensional vectors generated by training on extensive text corpora from Wikipedia and the web.  
%\textcolor{red}{The wide topic coverage of Wikipedia~\cite{Milne:06} ensures capturing the language use in the legal domain.} 
For computing the %To use this word-vector model for creating 
sentence embedding ($\vec{S}$), we first retrieve the corresponding embedding for each word in the sentence as given by the pre-trained model. Then, we average over all the word embeddings ($\vec{w_i}$) to get a single vector representing the sentence embedding.
\textcolor{blue}{Despite simplicity,  averaging and summation of embeddings have proved to be efficient compositional methods for generating sentence (or phrase) embeddings across a broad range of different domains and NLP tasks including text similarity~\cite{Wieting:15, Blacoe:12}. The objective of vectorization step in our approach is to get an effective, yet fast to train and test, representation for measuring text similarity.
we chose averaging because it outperformed summation in our experiments.  }
%That is, $\vec{S} = (\vec{w_1}.+\vec{w_2}.+\dots.+\vec{w_n})./n$, such that $.+$ and $./$ are element wise operations, and $n$ is the number of words in the sentence $S$.
For example, the embedding of the sentence ``data privacy policy'' in Fig.~\ref{fig:embeddings} is the average of the word embeddings in that sentence, such that the first entry in the sentence embedding (i.e., -0.14414) corresponds to the average of the first entries in the word embeddings of ``data'', ``privacy'', and ``policy'' (i.e., -0.47099, 0.099115, and -0.060532), respectively. 
%$\vec{S} = (\vec{w_1}.+\vec{w_2}.+\dots.+\vec{w_n})/n$

\begin{figure}[H]
\centering
\includegraphics[width=0.7\linewidth]  {img/step2}
\caption{Example of Vectorization.} \label{fig:embeddings}
%\vspace*{-1.7em}
\end{figure}

\subsubsection{ML-based Classification (Step~3)} %16 in total
In this step, we attempt to solve the multi-class multi-label classification problem by transforming it into multiple binary classification problems (as explained in Sec.~\ref{subsec:ml}). 
To do so, we apply the pre-trained %build
ML classifiers 
for predicting the presence of level-1 and level-2 metadata types in each sentence of the input privacy policy. 
We restrict the use of ML to level-1 and level-2 metadata types 
because the number of positive examples we have in our training set for level-3 is not sufficient for building accurate ML classifiers. 
Inspired by Wang and Manning~\cite{wang:12}, we use SVM with its default hyper-parameters for sentence classification.
%training
Our classifiers are trained on a feature matrix in which each row corresponds to a sentence and the columns are the 100-dimensional sentence embedding computed in step~2. The prediction class for each classifier indicates the presence of a level-1 or level-2 metadata type in the sentence. For example, the sentence ``Your personal data might be disclosed to the tax authorities, or other third parties including legal or financial advisors, regulatory bodies, auditors and technology providers.'' (number \textbf{14} in Fig.~\ref{fig:annotations}) is predicted as 
\textsc{Recipients}. 
We train the classifiers with positive examples representing the sentences that have been annotated with a particular metadata type (e.g., \textsc{Data Subject Right}) and negative examples annotated with any other metadata type \textit{at the same level} (e.g., all but \textsc{Data Subject Right}). 
In most of the cases, we obtained imbalanced datasets with positive examples being under-represented; this was addressed with under-sampling over negative examples~\cite{Witten:16}. \textcolor{blue}{Our preliminary experiments suggested that under-sampling outperformed   alternatives for handling imbalanced datasets (e.g., minority over-sampling and cost-sensitive classification). As we will discuss in Sec.~\ref{sec:evaluation}, The high accuracy obtained by our current solution  alleviates the need to empirically examine alternatives for handling imbalance.}

Step~3 uses one pre-trained binary classifier for each \hbox{level-1} and level-2 metadata type in the model of Fig.~\ref{fig:metadata}. 
% \textcolor{red}{using the filters provided in WEKA}.
The classifier predicts for each sentence in the input privacy policy, using its embedding vector as features, whether it should be labelled with the metadata type on which the classifier
has been trained. For example, the sentence ''the right to request erasure, restriction, portability, and to object to the processing of your personal data'' (numbers \textbf{29} -- \textbf{32} in Fig.~\ref{fig:annotations}) is predicted by the corresponding binary classifiers as the level-2 metadata types \textsc{Data Subject Right.\{Erasure, Restriction, Portability, and Object\}}. If a metadata type is not predicted by any classifier to be present in a sentence, then this metadata type is deemed as absent.  
The resulting classifications are passed on to step~6 (Prediction).
%We perform binary classification on level-1 and level-2 metadata types. 
%\textcolor{red}{Classifiers use the sentence embedding in the input privacy policy to determine whether the sentences refer to level-1 or level-2 metadata types.}

\subsubsection{Similarity-based Classification (Step~4)}
%In this step, we address level-2 of the metadata model in Fig.~\ref{fig:metadata}. 
In this step, we classify each sentence of the input privacy policy based on how similar it is to the group of sentences, in the training set, that are annotated with a certain level-1 or level-2 metadata type. % (e.g., \textsc{Data\_Subject\_Right.Access}). % as per the training set discussed in Sec.~\ref{subsection:annotation}. 
We restrict similarity-based classification method to level-1 and level-2 metadata types, because the number of positive examples for level-3 in our training set are not enough to produce conclusive results. %prompted by this type of classification not being conclusive enough for level-3, as observed in our experiments.
Similar to step~3, step~4 characterizes each sentence using the vector representation built in step~2.
%From the training set, we group the embeddings of the sentences that are annotated with a particular sub-metadata type.

Step~4 creates one group for each level-1 and level-2 metadata type. Since an individual sentence can have multiple metadata-type annotations, the same sentence embedding can be part of several groups.
%For each level-1 metadata type, this results in a number of sentence groups that is equal to its number of sub-metadata types in level-2 (e.g., eight groups represent level-2 metadata types of \textsc{Data\_Subject\_Right}), each of which labeled with the corresponding metadata name. 
Each group is represented by a single vector which is computed as the average of all sentence embeddings in that group. To predict whether a sentence ($S$) should be annotated with a certain %level-1 (or level-2) 
metadata type ($t$), we compute the \emph{cosine similarity} between the sentence embedding ($\vec{S}$) and the vector capturing the average embedding of the group of sentences annotated by $t$ (i.e., $\vec{t}$) in the training set. If the cosine similarity is above a pre-specified threshold, we predict $t$ to be a metadata type for $S$. \textcolor{blue}{More details about tuning this threshold will be provided in Sec.~\ref{sec:xx}.}
%We set the value of this threshold to 0.9. This value was empirically obtained by evaluating the accuracy of the prediction using a range of similarity threshold values between 0.5 and 0.9 with a step of 0.01 on a subset of the privacy policies in the training set. Threshold values less than 0.5 are not considered because they fail to capture the similarity. %, while values greater than 0.9 are already covered.
In our example in Fig.~\ref{fig:annotations}, the cosine similarity between the group of sentences that is annotated with %the level-2 metadata type 
\textsc{PD Origin.Indirect} ($t$) and the 
vector representation ($\vec{S}$) corresponding to sentence number \textbf{10}: ``information obtained from third parties including [...]'' is 0.91, while the similarity with $\vec{S^\prime}$ of sentence number \textbf{14}: ``Your personal data might be disclosed to the tax authorities, or other third parties [...]'' is  0.43. Therefore, $S$ is classified as $t$ while $S^\prime$ is not. The results of this step are passed on to step~6 (Prediction).
%~\cite{islam:08,bayardo:07}. 
%
%Next, we compute the cosine similarity between each sentence embedding in the input privacy policy and the average vector of each group. 
%If the sentence is found similar to a certain group, according to a set similarity threshold, then we label the sentence with the metadata name of the group. 
%The results of this step are passed over to Step 7 (Prediction).

\subsubsection{Keyword-based Classification (Step~5)}
%As explained in Sec.~\ref{subsection:annotation}, while annotating the privacy policies, 
%We developed a list of keywords for level-1, level-2 and level-3 metadata types. 
%We observed that the sentences referring to level-1 metadata types have less in common than those from level-2 and level-3 and, therefore, keeping keywords does not help at that level. 
In this step, we conduct a keyword search (from a predefined list) over the (textual) sentences in the input privacy policy. If a sentence $S$ contains one or more of the keywords associated with metadata type $t$, then we predict that $S$ should be annotated with $t$. 
For example, the sentences (number \textbf{38} and \textbf{39} in Fig.~\ref{fig:annotations}): ``[...] all \textbf{minors} who do use the website [...] obtained consent from the persons exercising \textbf{parental care} or from their \textbf{guardians}.'' will be predicted as \textsc{Children} because they contain keywords indicating this metadata type (highlighted in bold). 
As explained in
Sec.~\ref{sec:qualitative}, we have manually annotated 30 privacy policies that constitute a subset of our training set.
Using only these policies, we developed a list of keywords for \hbox{level-2} and level-3 metadata
types, collectively contain a total of 362 keywords. %We observed that the sentences referring to \hbox{level-1} metadata types have less in common than those from level-2 and level-3 and, therefore, using keywords would not be particularly helpful at that level.
%During our qualitative analysis (presented in Sec.~\ref{sec:qualitative} and Sec.~\ref{sec:criteria}), we have manually annotated 30 privacy policies in our training set. Using only these policies, we have created several lists of keywords, across level-2 and level-3 metadata types, that collectively contain a total of 525 keywords. 
\textcolor{blue}{Another important point in relation to keywords is that, the text generalization performed in step~1 improves the efficacy of keyword search for level-2 and level-3. For example, number \textbf{5} in Fig.~\ref{fig:annotations} represents an email address that is generalized with \textit{email}. Thus, including \textit{email} as a keyword enables identifying the metadata type \textsc{Contact.Email}. }
%The keywords will be made publicly available if the paper is accepted (see footnote 1 on page 1).
The results of this step (keyword search) are passed on to step~6 (Prediction).

%The same sentence might contain multiple metadata types originated from different level-1 due to overlapping KWs, e.g., the KW \textit{transfer} is a cue for both  \textsc{Data\_Subject\_Right.Portability} and \textsc{Transfer\_Outside\_Europe.Safeguards}. In this case, we keep the metadata types with the highest number of KWs if we find other KWs, otherwise we keep both metadata types.

%This step requires only the completion of the pre-processing step, as described in Fig.~\ref{fig:approach}. In other words, we do not need the word embedding of the sentence in this case. We check the presence of those words in sentences because this information might have been partially lost due to averaging the word embedding. 
%, which are the metadata names associated with each sentence according to the presence of KWs,

\subsubsection{Prediction (Step~6)}
This step combines the ML-based (step~3), similarity-based (step~4) and keyword-based (step~5) classification results to produce a final recommendation about which metadata types should be ascribed to a given sentence. 
\textcolor{blue}{The intuition behind using three different classification methods for predicting a hierarchical label is that each method alone has limitations but can give strong indications to a certain level. ML-based classifier can be used for predicting level-1 metadata types because we have enough many examples from which the classifier can learn. Using only ML-based for level-2 and level-3, however, is sufficient because for level-2 we have less examples so the ML-based classifier is not always accurate and therefore needs to be combined with another classification method. For level-3, ML cannot be used because we do not have enough examples. Our prediction step accounts also for the cases when ML-based missed a level-1 metadata type, but the other methods provide strong evidence for predicting level-2 metadata types.  }
%\textcolor{blue}{Level-1 can be predicted by ML-based or Similarity-based, level-2 metadata types can be predicted by all classifiers, and level-3 can be predicted by keyword-based only. 
%The possible combinations we present in this step for identifying level-1 and level-2 metadata types are centered primarily around ML- and similarity-based classification results because of the limitations of keyword-based classifier (discussed in Sec.~\ref{sec:introduction}). 
%}
Our strategy for combining the above classification methods is elaborated in Algorithm~\ref{alg}.
The algorithm starts with an initially empty set of hierarchical labels %annotations 
($\mathcal{M}$) -- \hbox{line 1}. A hierarchical label is represented as \textit{level-1.level-2.level-3}. Note that if the same label is predicted multiple times, only one copy is retained (since $\mathcal{M}$ is a set). 


\input{alg}

\sectopic{Level-1 and Level-2 Metadata.} 
\textcolor{blue}{The algorithm predicts a level-1 metadata type and its corresponding level-2 specializations in two cases. Case~1 applies when some \hbox{level-1} metadata type can be predicted, and then the algorithm attempts to predict its level-2. 
Case~2 applies when Case~1 fails to predict level-1 but there is still strong evidence for predicting its level-2 metadata type. 
Level-1 metadata types can be predicted by ML-based or similarity-based methods, whereas level-2 can be predicted by all classifiers. Due to the limitations of keywords (discussed in Sec.~\ref{sec:introduction}), they are used as complementary indicators for predicting level-2.}


\emph{\textbf{Case 1:}}
%The algorithm predicts a 
%level-1 metadata type ($\ell_i$) for a given sentence ($S$) if
%two supporting cues can be found. % in two cases (lines 3--6). The first case is 
%This is the case when  
\textcolor{blue}{If a level-1 metadata type ($\ell_i$) is predicted for the sentence ($S$) via the (level-1) ML-based classifier ($\mathit{cf}_1$) or by the similarity-based classifier
%, \textbf{and} further confirmed by keyword search (line 4), 
then $\ell_i$ is added to $\mathcal{M}$.
\textcolor{magenta}{ Our experiments discussed in Sec.~\ref{sec:evaluation} indicate that} ML-based  classifier provides strong indicators for distinguishing \hbox{level-1} metadata types. 
For each predicted $\ell_i$ that has any specialization, the algorithm attempts to further predict its level-2 metadata type ($\ell_j$). 
If $\ell_j$ is predicted by the (\hbox{level-2}) ML-based ($\mathit{cf}_2$), similarity-based or keyword-based classifiers (line 7), then the annotation $\ell_i.\ell_j$ is added to $\mathcal{M}$. Since $\ell_i$ has been confirmed earlier, it is sufficient to get the prediction about $\ell_j$ by one classifier. Regardless of whether or not the algorithm succeeds to predict $\ell_j$, $\ell_i$ is still added to $\mathcal{M}$ (line 5). The rationale is that pinpointing the sentence that discusses $\ell_i$ can help the legal experts more easily locate $\ell_j$ which is expected to appear in the following sentences.
}
%Prediction by the similarity-based classifier requires a similarity value between the sentence vector, $\vec{S}$, and the average vector of the associated group, $\vec{av}(\ell_i)$, to be above the threshold of 0.9. 
%If the algorithm confirms $\ell_i$ to be predicted for $S$ by the two methods as explained above, then $\ell_i$ is added to $\mathcal{M}$. 
%\sectopic{Level-2 Metadata.} 
%in two cases (lines 7--13). Given that its level-1 metadata type $\ell_i$ is already in $\mathcal{M}$, the first case is 
%when $\ell_j$ is predicted by both similarity-based classification (i.e., semantic similarity is above the threshold of 0.9) and keyword-based classification (line 9). In this case, $\ell_j$ is added to $\mathcal{M}$.

\emph{\textbf{Case 2: }}
\textcolor{blue}{The algorithm checks, for each level-1 metadata type ($\ell'_i$) that is not predicted in Case 1, whether its \hbox{level-2} ($\ell_j$) can still be predicted. Case~2 requires $\ell_j$ to be predicted by two classifiers. Specifically, if $\ell_j$ is predicted by the (\hbox{level-2}) ML-based ($\mathit{cf}_2$) and similarity-based classifiers (line 16), then the label $\ell'_i.\ell_j$ is added to $\mathcal{M}$. Alternatively, if $\ell_j$ is predicted by $\mathit{cf}_2$ or by the similarity-based classifier, and $\ell_j$ is further predicted by keyword search (line 18), then the label $\ell'_i.\ell_j$ is added to $\mathcal{M}$. In Case~2, $\ell'_i$ is automatically added to the set of annotations to get the hierarchical label, since there is enough evidence to support the prediction of $\ell_j$.} %Thus, both $\ell_i$ and $\ell_j$ are added to $\mathcal{M}$
%In the first case $\ell_j$ is added to $\mathcal{M}$ while in the second case both $\ell_i$ and $\ell_j$ are added to $\mathcal{M}$. Note that the second case covers the situation when $\ell_i$ is not predicted as level-1 metadata type due to the absence of evidence.
The level-2 metadata types \textsc{Controller.Identity} ($C_{ID}$) and \textsc{Controller Representative.Identity} ($CR_{ID}$) are provided %given
by the user through the questionnaire explained in Sec.~\ref{sec:criteria} (as answers to Q1 and Q5). \textcolor{blue}{If %one of these two metadata types (e.g.,\textsc{Controller.Identity}) 
$C_{ID}$ (or $CR_{ID}$) occurs in the sentence $S$, then \textsc{Controller.Identity} (or \textsc{Controller Representative.Identity}) %the corresponding hierarchical label
is added to $\mathcal{M}$ (lines 23 -- 27).
}


\sectopic{Level-3 Metadata.} The algorithm attempts to predict level-3 metadata types based on any already predicted level-1.level-2 annotation. Specifically, the algorithm considers all level-3 metadata types that specialize some level-2 metadata type already in $\mathcal{M}$. 
%Any considered 
For each level-2 metadata type that is predicted, if its level-3 %metadata type that 
is predicted by keyword search, then level-3 metadata type is added to $\mathcal{M}$ (line 31).

\subsubsection{Post-processing (Step~7)}
In the seventh and final step of our metadata identification approach, we refine the results of step~6 by considering the metadata types predicted for the sentences surrounding a given sentence. 
The intuition behind this step is the observation that specializations of certain metadata types are discussed in consecutive sentences of privacy policies.
Based on this observation, when a sentence $S$ is predicted as having a specific metadata type $t$, the surrounding context, specifically the preceding and succeeding sentences, can provide a confirmatory measure about whether $t$ is a reliable prediction for $S$.
%\textcolor{blue}{The number of sentences that we consider as potentially being in the same context depends on the number of metadata types at the same of $t$ and the previous level.} 

%level-2 metadata types in total. 

We employ several such context-based heuristics for post-processing. \textcolor{blue}{Specifically, \textsc{Data Subject Right}, \textsc{Transfer Outside Europe}, and \textsc{Legal Basis}. }
% listed next. %(not listed here due to space). 
%In relation to \textsc{Data Subject Right}, 
%we apply the following heuristic: 
\textcolor{blue}{The heuristic states that if some level-2 metadata type ($\ell_j$) %, which is a specialization of $\ell_i$ % --- a specialization of level-1 metadata type ($\ell_i$) --- 
is predicted for a sentence ($S$),  
%of \textsc{Data Subject Right} %$\mathit{DSR}_i$ 
%(e.g., \textsc{Data Subject Right.Access}), 
then we look at the $n+1$ %eight 
preceding and $n$ %eight 
succeeding sentences, such that $n$ equals the number of the metadata types at the same level of $\ell_j$, and $n+1$ accounts for the mention of $\ell_i$ preceding %prior discussing 
$\ell_j$.} \textcolor{blue}{For example, nine sentences (before) and eight (after) are considered to belong to the context for the level-2 metadata type \textsc{Data Subject Right.Portability}. The reason is that the eight other level-2 metadata types of \textsc{Data Subject Right} can be discussed (before or after), whereas \textsc{Data Subject Right} itself should have been discussed before. It makes no sense to discuss a level-2 prior to discussing level-1 metadata. 
}

If none of these surrounding sentences are predicted to be discussing a
 metadata type 
relevant to $\ell_j$, % (including $\ell_i$), %\textsc{Data Subject Right}
%$\mathit{DSR}_j$ 
%(e.g., \textsc{Data Subject Right.Erasure}), 
then we remove from the annotations for $S$ the predicted label that includes $\ell_j$. %\textsc{Data Subject Right} %$\mathit{DSR}_i$ 
This is because the context around $S$ lends no support to $\ell_j$ %\textsc{Data Subject Right} % $\mathit{DSR}_i$ 
being a correct annotation for~$S$. 
\textcolor{blue}{For example, the metadata type \textsc{Data Subject Right.Portability} can be falsely predicted for $S$ (sentence number \textbf{16} in Fig.~\ref{fig:annotations}), because of the misleading words (``transfer'', ``personal'', ``data'').
Then, we consider the \textit{nine} preceding (i.e., \textbf{7 -- 15}) and \textit{eight} following sentences (i.e., \textbf{17 -- 24}) to decide if there is  enough support to confirm the prediction of $S$, by looking at the presence of other metadata types relevant to \textsc{Data Subject Right.Portability}. }

\textcolor{blue}{We note that this step may filter out some correct annotations %if they happen to appear solely in a privacy policy, 
if there is not enough context supporting these annotations, e.g., when a privacy policy has only one sentence that discusses \textsc{Data Subject Right.Portability}, then it is likely that this annotation will be removed during post-processing. However, our experiments show that applying this step improves the prediction results.  } 

\subsection{Completeness Checking (Phase~B)}

Phase~B takes as an input: (1) the output of Phase~A representing the predicted metadata types in the input privacy policy, and (2) the answers of the user to the six questions discussed in Sec.~\ref{sec:criteria}. Phase~B then returns a detailed report 
of completeness analysis as the final output of our overall approach. 
This phase implements the completeness criteria depicted in Fig.~\ref{fig:Violations} and Fig.~\ref{fig:Warning}. 
Using our running example in Fig.~\ref{fig:annotations}, the expected answers to the questionnaire include \textit{Hikari Bank Ltd} as the \textsc{Controller.Identity} (\textbf{Q1)}, personal data will likely be transferred outside the EU %since the controller is in Japan
(\textbf{Q2}), there will be recipients other than the \textsc{Controller} (\textbf{Q3}), the core activities include processing special categories (\textbf{Q4}), processing of personal data will take place in Japan %Luxembourg and/or Japan
(\textbf{Q5}), and finally the personal data will be collected both directly and indirectly (\textbf{Q6}). The answer to \textbf{Q5} requires an additional input from the user about the \textsc{Controller Representative.Identity} which is \textit{the Holding Bank Services}.

Based on the answers given above, all completeness criteria (see Sec.~\ref{sec:criteria}) need to be checked in this step. 
For example, the criterion \textbf{C22} states that \textsc{PD Provision Obliged} should be present in a privacy policy when the legal basis of processing personal data is either \textsc{Legal Basis.Legal Obligation} or \textsc{Legal Basis.Contract.To Enter Contract}. A violation of this criterion %can 
raises an incompleteness issue.
In our example in Fig.~\ref{fig:annotations}, both the above-mentioned metadata types are found in the privacy policy, in sentences \textbf{20} and \textbf{25}, respectively. As a result, we have to find a mention of \textsc{PD Provision Obliged} in the same policy; this comes in sentence \textbf{26}. Had this sentence not been correctly identified by phase~A, either due to inaccurate prediction or because it is actually missing in the policy, then this criterion would have been violated.
The result of Phase~B is a %report that summarizes the
set of detected violations and warnings of the 23 criteria due to missing metadata in the input privacy policy.
%if the user answers question \textbf{Q2} as yes, then we should find the metadata type \textsc{Transfer Outside Europe}, and at least one specialization in level-2 and level-3 sub-metadata types, in the input privacy policy. Since the sentences ''We may also transfer your personal data to countries outside of European Union (including Japan) on the basis of: (i) European Commission’s adequacy decisions, certified by the APPI Japan scheme; (ii) our binding corporate rules; (iii) suitable standard contractual clauses.'' and ''By accepting this policy, you expressly consent the processing of your personal data by Hikari Bank and any of the group companies if fits or applies to a vacancy outside the European Union.'', contain information related to \textsc{Transfer Outside Europe} and all its level-2 and level-3 specializations, this requirement is fulfilled and thus, the compliance criteria C6, C7, C8, C9 and C10 result in no violations. 


==> casestudy.tex <==
\section{Case Study} \label{casestudy}

In this section, we describe the case study through which we answer RQ3 and RQ4. RQ3 aims to assess how accurate our automated metadata identification method is, whereas RQ4 aims to examine the accuracy of our overall approach for checking the completeness of privacy policies according to GDPR. We present our case study in terms of: (1) objectives and design (Sec.~\ref{subsec:CaseStudy}); (2) defining the completeness criteria of interest for the case study (Sec.~\ref{subsec:Criteria}); (3) identifying metadata in privacy policies (Sec.~\ref{subsec:Results});  and (4) checking the completeness of privacy policies (Sec.~\ref{subsec:Analysis}). 
\subsection{Objectives and Design}
\label{subsec:CaseStudy}
We evaluate our approach on the test set (as explained in Sec.~\ref{subsection:annotation}) with a total of 48 privacy policies that are not used during training or development.
\textcolor{red}{First we focus the evaluation on two metadata types:\textsc{Data Subject Right} (DSR) and \textsc{Legal Basis} (LB) and their descendants, based on their \textbf{importance} and \textbf{interdependence}. Then we performed the evaluation on all the remaining metadata types: \textsc{Transfer Outside Europe} (TOE), \textsc{PD Origin} (PDO), \textsc{PD Category} (PDC), \textsc{ReCipients} (RC), \textsc{PD Time Stored} (PDTS), \textsc{Processing Purposes} (PP), \textsc{PD Provision Obliged} (PDPO), \textsc{PD Security} (PDS), \textsc{Auto Decision Making} (ADM), \textsc{CHildren} (CH), \textsc{Data Protection Organization} (DPO), \textsc{ConTroller} (CT), \textsc{Controller Representative} (CR) and all their descendants (see Fig.~\ref{fig:metadata}).}

\textcolor{red}{In this section, we assess the accuracy of our approach in identifying all metadata types in privacy policies.} 
To measure accuracy, we use as gold standard the manually annotated versions of the 48 privacy policies in our test set. %\textcolor{red}{containing 625 sentences of DSR and 1418 sentences of LB}.
Our approach works at the sentence level, as explained in Sec.~\ref{extraction}. However, to answer RQ3, we need to evaluate the presence or absence of the metadata types of interest irrespectively of the number of sentences containing these metadata types. For example, if five sentences happen to discuss the metadata type \textsc{Data Subject Right.Access}, and at least one of them is correctly identified by our approach, then we consider this metadata type to be correctly identified for the underlying privacy policy.

This way of measuring accuracy is motivated by our objective, which is checking completeness; as can be seen from the criteria presented in Sec.~\ref{subsec:Criteria}, what one needs to ascertain to be able to verify the criteria is the presence or absence of the metadata types within an entire privacy policy.

To evaluate our metadata identification approach, we define: (1) \textit{True Positives (TPs)} to be the cases where at least one sentence is correctly identified for an expected metadata type according to the gold standard, (2) \textit{False Positives (FPs)} to be the cases where an incorrect metadata type is detected,  and (3) \textit{False Negatives (FNs)} to be the cases where we miss a metadata type that exists in the gold standard. 
\textcolor{red}{Following this definitions, we compute precision ($\mathit{TP} /(\mathit{TP} + \mathit{FP})$) and recall ($\mathit{TP} /(\mathit{TP} + \mathit{FN})$) across the test privacy policies for all the different metadata types.}

\begin{table}[!t]
\centering
\caption{Accuracy Results for Metadata Identification. } 
\footnotesize{
\begin{tabular}{p{1.7cm} c c l p{2.3cm} c c }
%\toprule
\cline{1-3} \cline{5-7}
\textbf{DSR}                                                & \textbf{P\%} & \textbf{R\%} &  & \textbf{LB}                                                          & \textbf{P\%} & \textbf{R\%} \\  %\cline{1-3} \cline{5-7}
\hhline{===~===}
\textsc{Access}                                                      & 98          & 96           &  & \textsc{Consent}                                                              & 100          & 95          \\ \cline{1-3} \cline{5-7} 
\textsc{Complaint}                                                    & 97          & 97          &  & \textsc{Contract}                                                             & 97           & 94           \\ \cline{1-3} \cline{5-7} 
\textsc{Complaint.SA}                                                & 97          & 100          &  & \textsc{Contract.To \-Enter~Contract} & 94          & 100           \\ \cline{1-3} \cline{5-7} 
\textsc{Erasure}                                                     & 100          & 98           &  & \textsc{Contract. \-Contractual}                                                 & 97           & 94          \\ \cline{1-3} \cline{5-7} 
\textsc{Object}                                                      & 100           & 97           &  & \textsc{Contract. Statutory}                                                   & 90           & 90          \\ \cline{1-3} \cline{5-7} 
\textsc{Portability}                                                 & 100          & 100          &  & \textsc{Legal \-Obligation}                                                     & 100          & 98           \\ \cline{1-3} \cline{5-7} 
\textsc{Rectification}                                               & 100          & 100           &  & \textsc{Legitimate \-Interest}                                                  & 100          & 91           \\ \cline{1-3} \cline{5-7} 
\textsc{Restriction}                                                 & 92          & 94           &  & \textsc{Public Function}                                                      & 100           & 90           \\ \cline{1-3} \cline{5-7} 
\textsc{Withdraw Consent} & 100          & 94           &  & \textsc{Vital \linebreak Interest}                                                       & 100          & 100           \\ \cline{1-3} \cline{5-7} 
\cline{1-3} \cline{5-7}
\textbf{TOE}                                                & \textbf{P\%} & \textbf{R\%} &  & \textbf{PDO}                                                          & \textbf{P\%} & \textbf{R\%} \\  %\cline{1-3} \cline{5-7}
\hhline{===~===}
\textsc{Specific Derogation}                                                      & 80          & 100           &  & \textsc{Direct}                                                              & 100           & 95          \\ \cline{1-3} \cline{5-7} 
\textsc{Safeguards}                                                    & 92          & 100          &  & \textsc{Indirect}                                                             & 98           & 100           \\ \cline{1-3} \cline{5-7} 
\textsc{Adequacy Decision}                                                & 100          & 100          &  & \textsc{Indirect. Third Party} & 94          & 100           \\ \cline{1-3} \cline{5-7} 
\textsc{Specific Derogation.Unambiguous Consent}                                                     & 75           & 100           &  & \textsc{Indirect.Publicly}                                                 & 96           & 100          \\ \cline{1-3} \cline{5-7} 
\textsc{Safeguards. Binding Corporate Rules}                                                      & 100           & 100           &  & \textsc{Indirect.Cookie}                                                   & 90           & 93          \\ \cline{1-3} \cline{5-7} 
\textsc{Safeguards. EU Model Clauses}                                                 & 87          & 100          &  & \textbf{PDC}                                        & \textbf{P\%} & \textbf{R\%}           \\ \cline{1-3} \cline{5-7} 
\hhline{~~~~===}
\textsc{Adequacy Decision. Territory}                                               & N/A           & N/A           &  & \textsc{Special}                                                  & 90           & 100           \\ \cline{1-3} \cline{5-7} 
\textsc{Adequacy Decision. Sector}                                                 & N/A           & N/A           &  & \textsc{Type}                                                      & 75           & 100           \\ \cline{1-3} \cline{5-7} 
\textsc{Adequacy Decision. Country} & 100          & 100           &  & \textsc{}                                                       &            &            \\ \cline{1-3} \cline{5-7} 
\textbf{DPO}                                                & \textbf{P\%} & \textbf{R\%} &  & \textbf{Metadata}                                                          & \textbf{P\%} & \textbf{R\%} \\  %\cline{1-3} \cline{5-7}
\hhline{===~===}
\textsc{Contact}                                                      & 92          & 92           &  & \textsc{Recipients}                                                              & 100           & 100          \\ \cline{1-3} \cline{5-7} 
\textsc{Contact.Phone Number}                                                      & 100          & 100           &  & \textsc{PD Time Stored}                                                              & 97           & 100          \\ \cline{1-3} \cline{5-7} 
\textsc{Contact.Email}                                                    & 96          & 96          &  & \textsc{PD Provision Obliged}                                                             & 100           & 84           \\ \cline{1-3} \cline{5-7} 
\textsc{Contact.Legal Address}                                                & 83          & 88          &  & \textsc{Processing Purposes} & 100          & 100           \\ \cline{1-3} \cline{5-7} 
\textbf{Metadata}                                                     & \textbf{P\%} & \textbf{R\%}           &  & \textsc{PD Security}          & 98          & 100                            \\ \cline{1-3} \cline{5-7} 
\hhline{===~}
\textsc{Auto Decision Making}                                                     & 88           & 96           &  & \textsc{Children}                 & 75           & 90                \\ \cline{1-3} \cline{5-7}
\textbf{CT}                                                & \textbf{P\%} & \textbf{R\%} &  & \textbf{CR}                                                          & \textbf{P\%} & \textbf{R\%} \\  %\cline{1-3} \cline{5-7}
\hhline{===~===}
\textsc{Identity}                                                      & 100          & 100           &  & \textsc{Identity}                                                              & 100           & 100          \\ \cline{1-3} \cline{5-7} 
\textsc{Contact}                                                    & 97          & 97          &  & \textsc{Contact}                                                             & 100           & 67           \\ \cline{1-3} \cline{5-7}
\textsc{Identity.Legal Name}                                                & 100          & 100          &  & \textsc{Identity.Legal Name} & 100          & 100           \\ \cline{1-3} \cline{5-7} 
\textsc{Identity.Register Number}                                                & 75          & 75          &  & \textsc{Identity.Register Number} & 100          & 100           \\ \cline{1-3} \cline{5-7} 
\textsc{Contact.Phone Number}                                                     & 86          & 92           &  & \textsc{Contact.Phone Number}                                                 & N/A           & N/A          \\ \cline{1-3} \cline{5-7} 
\textsc{Contact.Email}                                                      & 95           & 87           &  & \textsc{Contact.Email}                                                   & N/A           & N/A          \\ \cline{1-3} \cline{5-7} 
\textsc{Contact.Legal Address}                                                 & 96          & 93          &  & \textsc{Contact.Legal Address}                                                     & 100          & 67           \\ \cline{1-3} \cline{5-7} 
\end{tabular}}
\label{tab:metrics}
%\vspace*{-1.7em}
\end{table}

\textcolor{red}{Table~\ref{tab:metrics} reports the accuracy of metadata identification for DSR and LB. As shown by the table, our approach have a precision and recall greater or equal to 94\% for almost all the metadata types, except for \textsc{Restriction}, with a precision of 92\%. The approach achieve the perfection for two out of the eight DSR level-2 metadata types, these are \textsc{Portability} and \textsc{Rectification}.}

\textcolor{red}{Achieving high precision implies that our approach is able to correctly identify the metadata types considered with zero or very few FPs. In the case of DSR, the metadata types \textsc{Access}, \textsc{Complaint} and \textsc{Complaint.SA} the approach produces one FP alongside with the 43, 38 and 36 correct identifications of each metadata. Also for \textsc{Restriction} metadata type, the approach has three FP alongside with the 33 correct identifications. Similarly, a high recall implies that our approach does not miss any instance of the metadata or miss very few of them. For the metadata types \textsc{Access}, \textsc{Restriction} and \textsc{Withdraw Consent}, the approach yields two FNs each and in the case of \textsc{Complaint}, \textsc{Erasure} and \textsc{Object} has only one respectively.}

\textcolor{red}{For LB, our approach yields a precision of 100\% for all the level-2 except for \textsc{Contract} with a 97\%. In the case of the level-3 metadata types, the three of them have a precision greater or equal to 94\%. Also, a good recall is obtained for all these metadata types, being greater or equal to 90\% in all cases. Here, the lower values are for \textsc{Contract$.$Statutory} and \textsc{Public Function}. Regarding these two metadata types, we note that these are rare in the fund domain. We, therefore, have few examples in our experimental material (both for training and development and for testing). As expected, the accuracy of our approach is lower for these metadata types.}

\textcolor{red}{Table~\ref{tab:metrics} also reports the accuracy of metadata identification for TOE, PDO and PDC. As shown by the table, our approach achieves a perfect precision for three out of nine TOE level-2 and level-3 metadata types and a perfect recall for seven of them. In the case of the level-3 metadata types \textsc{Adequacy Decision.Sector} and \textsc{Adequacy Decision.Territory}, we have not been able to find any example in our experimental material (both for training and development and for testing). Thus, it is not possible for us to compute any result about these two metadata types.}

\textcolor{red}{ For PDO and PDC metadata types, the approach achieve a precision grater or equal to 90\% except for \textsc{Type} with 75\%. In the case of recall, the approach yields a perfect recall for five out of seven metadata types. It is just not able to achieve this for \textsc{Direct} (95\%) and \textsc{Indirect.Cookie} (93\%), producing 2 FNs each along with 38 and 26 correct identifications of these metadata, respectively.}

\textcolor{red}{Similarly, Table~\ref{tab:metrics} reports the accuracy of metadata identification for DPO and its sub metadata types, RC, PDTS, PP, PDPO, PDS, ADM and CH. As shown by the table, our approach achieves a precision grater to 96\%, for almost all the independent metadata types, only \textsc{Children} with 75\% and \textsc{Auto Decision Making} with 88\% are out of this achievement. In the case of recall, the approach yield the perfection in four out out of seven independent metadata types. Here the metadata types \textsc{PD Provision Obliged}, \textsc{Children} and \textsc{Auto Decision Making} have 84\%, 90\% and 96\%, respectively. Concerning DPO, the table shows that for these metadata types, precision and recall have a range between 83\% and 100\%, achieving the perfection only in \textsc{Contact.Phone Number}. As it can be seen, the precision, in the case of \textsc{Children} is lower than for the other metadata types. This is due to the very few examples existing, as part of our experimental material. Our approach leads to three FPs over this metadata.}

\textcolor{red}{Finally, Table~\ref{tab:metrics} reports the accuracy of metadata identification for CT and CR. In the table, it is shown that the approach achieves a precision and recall grater or equal to 86\% for all the CT level-2 and level-3 metadata types, except for \textsc{Identity.Register Number} with 75\% in all metrics, having one FP and one FN. For the CT metadata types, the approach yields in total six FPs and eight FNs alongside with 136 correct predictions. In the case of CR, it can be seen that the precision and recall are perfect for almost all of the level-2 and level-3 metadata types, and that there exist no instances of two of them, which makes it impossible to compute any result for these last ones. As it can be seen, the recall, in the case of \textsc{Contact.Legal Address}, is significantly lower than for the other CR metadata types. This is because the sentences containing these metadata, do not follow the expected pattern to recognize, that is, these sentences do not meet certain predefined requirement.}

\textcolor{red}{\textbf{The answer to RQ3 is}: Our approach achieves an average precision of 98\%, 98\%, 91\%, 96\%, 95\%, 100\%, 97\%, 100\%, 100\%, 98\%, 88\%, 75\%, 92\%, 96\%, 100\% and an average recall of 97\%, 94\%, 100\%, 98\%, 100\%, 100\%, 100\%, 84\%, 100\%, 100\%, 96\%, 90\%, 93\%, 94\%, 80\% for \textsc{Data Subject Right}, \textsc{Legal Basis}, \textsc{Transfer Outside Europe}, \textsc{PD Origin}, \textsc{PD Category}, \textsc{ReCipients}, \textsc{PD Time Stored}, \textsc{PD Provision Obliged}, \textsc{Processing Purposes}, \textsc{PD Security}, \textsc{Auto Decision Making}, \textsc{CHildren}, \textsc{Data Protection Organization}, \textsc{ConTroller} and \textsc{Controller Representative}, respectively. It can be seen that all the metadata types have a precision over 90\% except for \textsc{Auto Decision Making} with an 88\% and \textsc{CHildren} with 75\%. Similarly, the only metadata types with recall below 90\% are \textsc{PD Provision Obliged} with 84\% and \textsc{Controller Representative} with 80\%.} 

\subsection{Completeness Checking of Privacy Policies (RQ4)} 
\label{subsec:Analysis}
While the accuracy of metadata identification has a direct influence on the accuracy of completeness checking, RQ3 per se does not measure the accuracy of completeness checking; this is instead the subject of RQ4.

%In this section, we discuss how our metadata identification approach can be used for identify incompleteness issues in  privacy policies.
%We focus on the privacy policies found to be incomplete by our approach. 
To answer RQ4, we need to redefine TP, FP, and FN in the context of completeness checking. Specifically, we define: (1)~\textit{TPs} as cases where the approach correctly identifies a genuine violation of some completeness criterion, (2) \textit{FPs} as cases where some criterion that is actually satisfied by the policy is incorrectly found to be violated, and (3) \textit{FNs} as cases where there is actually a violation of some criterion but this violation goes undetected by our approach.

\begin{table}[]
\centering
\caption{Accuracy Results for Incompleteness Detection. }\label{tab:analysis}
\begin{tabular}{ l l l l | l l }
\hline
\textbf{\#}  & \textbf{TPs} & \textbf{FPs} & \textbf{FNs} & \textbf{P\%} & \textbf{R\%} \\ \hline\hline
\textbf{C1}  & 14           & 1            & 1            & 93           & 93          \\ \hline
\textbf{C2}  & 2            & 0            & 1           & 100           & 67         \\ \hline
\textbf{C3}  & 4            & 1            & 0           & 80           & 100         \\ \hline
\textbf{C4}  & 7            & 1            & 2           & 88           & 78          \\ \hline
\textbf{C5}  & 12           & 2            & 1            & 86           & 92          \\ \hline \hline
\textbf{C6}  & 8           & 0            & 0            & 100           & 100          \\ \hline \hline
\textbf{C7}  & 5           & 0            & 0            & 100           & 100          \\ \hline \hline
\textbf{C8}  & 1           & 0            & 0            & 100           & 100          \\ \hline \hline
\textbf{C9}  & 2           & 0            & 1            & 100           & 67          \\ \hline \hline
\textbf{C10}  & 4           & 0            & 0            & 100           & 100          \\ \hline \hline
\textbf{C11}  & 5           & 0            & 1            & 100           & 83         \\ \hline \hline
\textbf{C12}  & 7           & 0            & 0            & 100           & 100        \\ \hline \hline
\textbf{C13}  & 2           & 0            & 0            & 100           & 100         \\ \hline \hline
\textbf{C14}  & 33           & 1            & 1            & 97           & 97         \\ \hline \hline
\textbf{C15}  & 2           & 0            & 0            & 100           & 100         \\ \hline \hline
\textbf{C16}  & 9           & 0            & 1            & 100           & 90          \\ \hline \hline
\textbf{C17}  & 23           & 4            & 0            & 85           & 100         \\ \hline \hline
\textbf{C18}  & 2           & 0            & 0            & 100           & 100         \\ \hline \hline
\textbf{C19}  & 22           & 2            & 2            & 92           & 92         \\ \hline \hline
\textbf{C20}  & 2           & 0            & 0            & 100           & 100         \\ \hline \hline
\textbf{C21}  & 16           & 1           & 1           & 94            & 94         \\ \hline \hline
\textbf{C22}  & 18           & 0            & 0            & 100            & 100          \\ \hline \hline
\textbf{C23}  & 18           & 1            & 0            & 95           & 100         \\ \hline \hline
\textbf{Summary} & \textbf{218}  & \textbf{14}   & \textbf{12}   & \textbf{94}  & \textbf{95}  \\ \hline
\end{tabular}
%\vspace*{-0.4em}
\end{table}

\textcolor{red}{In Tab.~\ref{tab:analysis}, we show our accuracy results for completeness checking. We have organized the results in this table according to the criteria, C1-C22, presented in Sec.~\ref{subsec:Criteria}. Below, we discuss the results for all of the 22 criteria.}

\textcolor{red}{\noindent\textbf{C1, C3, C4, C13, C18, C20:} 
104 genuine out of 112 incompleteness issues are detected along with eight FPs. These FPs are caused by the metadata identification phase having missed \textsc{DPO.Contact} metadata type twice, \textsc{Access} and \textsc{Restriction} once, \textsc{Erasure} and \textsc{Withdraw Consent} once, when the metadata type \textsc{Consent} was present, \textsc{Object} once, when at least one of the metadata types \textsc{Legitimate Interest} or \textsc{Public Function} was present, also \textsc{Type} and \textsc{CT.Contact} once.}

\textcolor{red}{\noindent\textbf{C5, C6, C7, C9, C11, C12, C14, C17, C19, C21, C22:} All the 69 actual incompleteness issues are detected with no FPs nor missing issues.}

\textcolor{red}{\noindent\textbf{C2, C16:} 27 actual incompleteness issues are detected along with five FPs. The FPs are caused by the metadata identification phase having missed the metadata type \textsc{Portability} when \textsc{Contract} was present and four times \textsc{PD Provision Obliged}.}

\textcolor{red}{\noindent\textbf{C8, C10, C15:} 16 actual incompleteness issues are detected and three missing. The missed issues stem from the metadata identification phase, incorrectly detecting the presence of the metadata types \textsc{Safeguards}, \textsc{Indirect} and \textsc{PD Time Stored} once each, which resulted in missing incompleteness issues. There are no FPs for these criteria.}

When checking the completeness of privacy policies, recall is more important than precision. This is because a human analyst can dismiss the FPs (false alarms) with relative ease as long as there are not too many of them. On the other hand, a deficit in recall means that the automation is missing incompleteness issues. Unless recall is very high, an expert is thus unlikely to trust the automatically generated results and may opt for a fully manual analysis.

\textcolor{red}{At a privacy-policy level, although the approach did not have perfect recall on C1, C2, C4, C5, C9, C11, C14, C16, C19 and 21, it is able to correctly identify that exist at least one incompleteness issue on each privacy policy in the test set. This means that no incomplete policy could pass through our approach undetected. Similarly, although the approach did not have perfect precision on C1, C3, C4, C5, C14, C17, C19, C21 and C23 no false incompleteness alarm is rising in any privacy policy.} 

%Note that the number of incomplete privacy policies presented along the results of the criteria does not add up to 12, since %, as it often happens, 
%multiple criteria can be violated in the same privacy policy. For example, a privacy policy that violates C1, can also violate C2, C3 or C4. 

\textcolor{red}{\textbf{The answer to RQ4 is}: Our approach is able to detect 218 out of the total of 230 incompleteness issues in the 48 privacy policies in our test set. Over these policies, the approach had 14 false positives. The approach thus has a precision and recall of 94\% and 95\%, respectively, over our case study. At the level of policies, the approach could correctly identify all the inconsistencies in 40 out of the 48 privacy policies.} 

\subsection{Completeness Criteria}
\label{subsec:Criteria}

\begin{table}[t!]
\begin{tabular}{p{1.0cm} p{1.5cm} p{5.2cm}}
\hline 
\textbf{Criteria} & \textbf{Reference} & \textbf{Intuitive Description}    
            \\ \hline\hline 

\textsc{C1}               & Art.~13.2(b), 13.2(d), 14.2(c), 14.2(e) and 21.4       & The DSR sub-metadata types \textsc{Access, Complaint, Rectification}, and \textsc{Restriction}, must be present. \\ \hline

\textsc{C2}               & Art. 13.2(d) and 14.2(e)            & If the DSR sub-metadata type \textsc{Complaint} is present, then the sub-metadata type \textsc{SA} should be present. \\ \hline

\textsc{C3}               & Art. 13.2(b), 14.2(c). 21.4            & If the LB sub-metadata type \textsc{Contract} is present, then the DSR sub-metadata type \textsc{Portability} should be present. \\ \hline

\textsc{C4}            & Art. 13.2(b), 14.2(c). 21.4            & If either of the LB sub-metadata types \textsc{Legitimate Interest} or \textsc{Public Function} are present, then the DSR sub-metadata type \textsc{Object} should be present. \\ \hline

\textsc{C5}               & Art. 13.2(b), 13.2(c), 14.2(c), 14.2(d), 7 and 21.4            & If the LB sub-metadata type \textsc{Consent} is present, then the DSR sub-metadata types \textsc{Erasure, Object, Portability}, and \textsc{Withdraw Consent} should be present. \\ \hline

\textsc{C6}               & Art. 13.1(f) and 14.1(f)       & The TOE metadata type should be present. \\ \hline

\textsc{C7}               & Art. 13.1(f) and 14.1(f)       & If the TOE metadata type is present, then at least one of the TOE sub-metadata types \textsc{Adequacy Decision, Safeguards, Specific Derogation}, should be present. \\ \hline

\textsc{C8}               & Art. 13.1(f) and 14.1(f)       & If the TOE sub-metadata type \textsc{Specific Derogation} is present, then its sub-metadata type \textsc{Unambiguous Consent}, should be present. \\ \hline

\textsc{C9}               & Art. 13.1(f) and 14.1(f)       & If the TOE sub-metadata type \textsc{Safeguards} is present, then at least one of its sub-metadata types \textsc{EU Model Clauses, Binding Corporate Rules}, should be present. \\ \hline

\textsc{C10}               & Art. 13.1(f) and 14.1(f)       & If the TOE sub-metadata type \textsc{Adequacy Decision} is present, then at least one of its sub-metadata types \textsc{Territory, Sector, Country}, should be present. \\ \hline

\textsc{C11}               & Art. 14.2(f)       & The PDO sub-metadata type \textsc{Indirect} should be present. \\ \hline

\textsc{C12}               & Art. 14.2(f)       & If the PDO sub-metadata type \textsc{Indirect} is present, then at least one of its sub-metadata types \textsc{Third Party, Publicly}, should be present. \\ \hline

\textsc{C13}               & Art. 14.1(d)       & The PDC metadata type should be present. \\ \hline

\textsc{C14}               & Art. 14.1(d)       & If either of the PDO sub-metadata types \textsc{Third Party} or \textsc{Publicly} are present, then the PDC sub-metadata type \textsc{Type}, should be present. \\ \hline

\textsc{C15}               & Art. 13.1(e) and 14.1(e)       & The RC metadata type should be present. \\ \hline

\textsc{C16}               & Art. 13.2(a) and 14.2(a)       & The PDTS metadata type must be present. \\ \hline

\textsc{C17}               & Art. 13.1(c) and 14.1(c)       & The PP metadata type must be present. \\ \hline

\textsc{C18}               & Art. 13.2(e)       & If either of the LB sub-metadata types \textsc{To Enter Contract} or \textsc{Legal Obligation} are present, then the PDPO metadata type should be present. \\ \hline

\textsc{C19}               & Art. 13.1(a) and 14.1(a)       & At least one of the \textsc{Contact} sub-metadata types \textsc{Legal Address, Email, Phone Number}, of DPO, should be present. \\ \hline

\textsc{C20}               & Art. 13.1(a) and 14.1(a)       & The CT sub-metadata type \textsc{Identity} must be present. \\ \hline

\textsc{C21}               & Art. 13.1(a) and 14.1(a)       & At least one of the \textsc{Contact} sub-metadata types \textsc{Legal Address, Email, Phone Number}, of CT, must be present. \\ \hline

\textsc{C22}               & Art. 13.1(a) and 14.1(a)       & The CR sub-metadata type \textsc{Identity} should be present. \\ \hline

\textsc{C23}               & Art. 13.1(a) and 14.1(a)       & At least one of the \textsc{Contact} sub-metadata types \textsc{Legal Address, Email, Phone Number}, of CR, should be present. \\ \hline

\end{tabular}
%\vspace*{-1.7em}
\end{table}



==> discussion.tex <==
\sectopic{Discussion.} 

As discussed in RQs, our approach achieves an average precision of $\approx$92\% and a recall of $\approx$95\% in identifying the mentions of different metadata types in a given privacy policy and consequently checks for completeness with a precision of $\approx$93\% and a recall of $\approx$90\%. 
The practical impact of using our approach is a significant .   

At a privacy level.
%48 privacy policies
\iffalse
currently all are incomplete  
Artemis, AshMore, BHPLS, Bluebay, Dpam-Charte, Erste, ING, Lombard => complete with warnings?
Edgewood, Putnam => complete without warnings? 
\fi

==> keywords.tex <==
Legal Compliance
Privacy Policies
The General Data Protection Regulation
Natural Language Processing
Machine Learning
Case Study Research

